Online Continual Learning via Logit Adjusted Softmax

Online continual learning is a challenging problem where models must learn from a non-stationary data stream while avoiding catastrophic forgetting. Inter-class imbalance during training has been identified as a major cause of forgetting, leading to model prediction bias towards recently learned classes. In this paper, we theoretically analyze that inter-class imbalance is entirely attributed to imbalanced class-priors, and the function learned from intra-class intrinsic distributions is the Bayes-optimal classifier. To that end, we present that a simple adjustment of model logits during training can effectively resist prior class bias and pursue the corresponding Bayes-optimum. Our proposed method, Logit Adjusted Softmax, can mitigate the impact of inter-class imbalance not only in class-incremental but also in realistic general setups, with little additional computational cost. We evaluate our approach on various benchmarks and demonstrate significant performance improvements compared to prior arts. For example, our approach improves the best baseline by 4.6% on CIFAR10.

==> contents/g_limitation.tex <==
\section{Limitation}
\label{sec:implication and limitation}
 As the focus of our proposed method in this paper is primarily on addressing the impact of inter-class imbalance and forgetting induced by recency bias on CL performance. We eliminate the imbalanced class-priors to improve performance. However, it can not provide any benefits when faced with domain-IL scenarios with only intra-class domain drift and no inter-class imbalance. One of our next research focuses is to develop task-free domain-IL methods to efficiently address intra-class domain drift. We hope to integrate our method with task-free domaim-IL methods to form a comprehensive solution for online general CL.

==> contents/tables/BCL.tex <==
\begin{table*}[htb]
        \caption{AUC of Accuracy $A_{\text{AUC}}$ and final average accuracy $A_T$ (both higher is better) on B-CIFAR100 (10 tasks) and B-TinyImageNet (10 tasks) with disjoint ratio $N_{\text{blurry}}=50$ and blurry level $M_{\text{blurry}}=10$. We show the results of top-3 methods. Memory sizes are $M=2k$.}
        \label{tab:blurry cl}
        \centering
        \begin{tabular}{@{}l | c | c@{}} 
        \toprule
        \textbf{Dataset}             & B-CIFAR100                   & B-TinyImageNet\\
        \midrule
        \textbf{Method}              &  $A_{T}\uparrow$ / $A_{\text{AUC}}\uparrow$   & $A_{T}\uparrow$ / $A_{\text{AUC}}\uparrow$ \\
        % \midrule
        \midrule
        ER   &\small$19.6$\tiny{$\pm1.6$}\small{$/$}\small$16.1$\tiny{$\pm0.1$} &\small$16.2$\tiny{$\pm0.2$}\small{$/$}\small$12.4$\tiny{$\pm0.0$}\\
        ER-ACE       &\small$18.3$\tiny{$\pm1.0$}\small{$/$}\small$15.2$\tiny{$\pm0.0$} &\small$16.4$\tiny{$\pm0.3$}\small{$/$}\small$12.2$\tiny{$\pm0.1$}\\
        CLIB         &\small$21.9$\tiny{$\pm0.3$}\small{$/$}\small$18.0$\tiny{$\pm0.1$} &\small$15.9$\tiny{$\pm0.2$}\small{$/$}\small$12.6$\tiny{$\pm0.1$}\\
        \rowcolor{myblue}
        ER-LAS              &\small$\mathbf{24.9}$\tiny{$\mathbf{\pm0.5}$}\small{$/$}\small$\mathbf{20.3}$\tiny{$\mathbf{\pm0.0}$} &\small$\mathbf{19.4}$\tiny{$\mathbf{\pm0.4}$}\small{$/$}\small$\mathbf{15.1}$\tiny{$\mathbf{\pm0.0}$} \\
        \bottomrule
        \end{tabular}
\end{table*}


==> contents/tables/CIL_large.tex <==
\begin{wraptable}{r}{0.45\columnwidth}
\vspace{-20pt}
\caption{Final average accuracy $A_T$ (higher is better) and final average forgetting $F_T$ (lower is better) on C-ImageNet (90 tasks) and C-iNaturalist (26 tasks). We show the results of top-3 methods. Memory sizes are $M=20k$.}
\label{tab:imagenet-inat}
\centering
\resizebox{0.45\columnwidth}{!}{
\begin{tabular}{@{}l|c|c@{}}
      \toprule
      \textbf{Dataset} & C-ImageNet                      & C-iNaturalist \\
      \midrule
      \textbf{Method}  & $A_T\uparrow$ / $F_T\downarrow$         & $A_T\uparrow$ / $F_T\downarrow$ \\
      \midrule
      ER & \small$31.8$\tiny{$\pm0.1$} \small{$/$} \small$38.6$\tiny{$\pm0.2$}                        & \small$4.7$\tiny{$\pm0.0$} \small{$/$} \small$18.0$\tiny{$\pm0.0$}  \\
      ER-ACE & \small$33.4$\tiny{$\pm0.2$} \small{$/$} \small$11.3$\tiny{$\pm0.1$}                    & \small$5.7$\tiny{$\pm0.0$} \small{$/$} \small$1.1$\tiny{$\pm0.0$}  \\ 
      MRO & \small$35.8$\tiny{$\pm0.1$} \small{$/$} \small$10.2$\tiny{$\pm0.2$}                     & \small$5.0$\tiny{$\pm0.0$} \small{$/$} \small$\bf{0.4}$\tiny{$\bf{\pm0.0}$}  \\
      \rowcolor{myblue}
      ER-LAS & \small$\bf{39.3}$\tiny{$\bf{\pm0.1}$} \small{$/$} \small$\bf{9.0}$\tiny{$\bf{\pm0.1}$}                     & \small$\bf{8.1}$\tiny{$\bf{\pm0.0}$} \small{$/$} \small$2.8$\tiny{$\pm0.0$}  \\
      \bottomrule
\end{tabular}}
\vspace{-10pt}
\end{wraptable}

==> contents/tables/CIL_mitigation.tex <==
\begin{table*}[b]
    \caption{\textbf{Response to W3\&Q5 of Reviewer Fvg4}. Comparison of final average accuracy by ER, ER-LAS, and imbalance mitigation methods. Experimental settings are the same as in Table 1 of the manuscript. Memory sizes are $M=1k$.}
    \label{tab:A}
    \centering
    \begin{tabular}{@{}l | c | c | c@{}} 
    \toprule
    \textbf{Dataset}         &C-CIFAR10&C-CIFAR100&C-TinyImageNet\\
    \midrule
        ER [13]&$45.4\pm1.8$ &$16.5\pm0.4$  &$11.0\pm0.2$\\
        ER-CBL [17]&$48.1\pm1.6$ &$18.8\pm0.2$  &$11.1\pm0.2$\\
        ER-WN [18]&$46.1\pm1.5$ &$16.6\pm0.8$  &$11.0\pm0.1$\\
        ER-Up [19]&$53.6\pm1.6$ &$23.4\pm0.5$  &$15.0\pm0.1$\\
        ER-Down [19]&$48.2\pm1.6$ &$18.9\pm0.3$  &$13.4\pm0.2$\\
        \rowcolor{myblue}
        ER-LAS&$\mathbf{55.3\pm1.6}$ &$\mathbf{25.7\pm0.3}$  &$\mathbf{15.5\pm0.2}$\\
    \bottomrule
    \end{tabular}
\end{table*}
